Mitigating Transient Bullwhip Effects Under Imperfect Demand Forecasts

Motivated by how forecast errors exacerbate order fluctuations in supply chains, we leverage robust feedback controller synthesis to characterize, compute, and minimize the worst-case order fluctuation experienced by an individual supply chain vendor. Assuming bounded forecast errors and demand fluctuations, we model forecast error and demand fluctuations as inputs to linear inventory dynamics, and use the $\ell_\infty$ gain to define a transient Bullwhip measure. In contrast to the existing Bullwhip measure, the transient Bullwhip measure explicitly depends on the forecast error. This enables us to separately quantify the transient Bullwhip measure's sensitivity to forecast error and demand fluctuations. To compute the controller that minimizes the worst-case peak gain, we formulate an optimization problem with bilinear matrix inequalities and show that it is equivalent to minimizing a quasi-convex function on a bounded domain. We simulate our model for vendors with non-zero perishable rates and order backlogging rates, and prove that the transient Bullwhip measure can be bounded by a monotonic quasi-convex function whose dependency on the product backlog rate and perishing rate is verified in simulation.

==> supply_chain_w_forecast.tex <==
\section{LTI/LQR model of supply chain with forecast}
From Udenio's paper~\cite{udenio2017behavioral}.
Consider a linear time invariant system with the following components for modeling a single product retailer.
\begin{enumerate}
    \item \textbf{Inventory} $i_t \in \reals$: amount of inventory at time $T$.
    \item \textbf{Pipeline} $p^{j}_t\in\reals$: amount of product projected to arrive at $t+j$, $j \in [1,\ldots L]$
    \item \textbf{Forecast} $f_t \in \reals$: forecasted demand for demand $t+1$.
    \item \textbf{Order} $o_t \in \reals$: amount ordered at time $t$.
    \item \textbf{Demand} $d_t \in\reals$: demand amount at time $t$
\end{enumerate}
If we ignore the fact that inventory, pipeline and orders cannot be negative. We can derive the following LTI system 
\begin{equation}\label{eqn:lti_system}
    \begin{bmatrix}
        i\\ p^1 \\ \vdots\\ p^L \\ f 
    \end{bmatrix}_{t+1} = \begin{bmatrix}
        1 & 1 &\ldots &0\\
        0& 0& \ldots & 0\\
        & &\ddots& \\
        0& \ldots& 0&1\\
        0& 0&\ldots&\alpha
    \end{bmatrix}\begin{bmatrix}
        i\\ p^1 \\ \vdots\\ p^L \\ f 
    \end{bmatrix}_t - \begin{bmatrix}
        0\\ \vdots\\ 0\\1 \\ 0
    \end{bmatrix}o_t - \begin{bmatrix}
        1 \\ 0\\ \vdots \\ 1 - \alpha
    \end{bmatrix}d_t, \quad \forall t \in \mathbb{N}, \ \alpha \in (0,1)s
\end{equation}
The resulting system matrix is $A$ is upper triangular as well as Jordan form. Therefore without control or disturbance, the dynamics is always marginally stable with eigenvalues $1$ and $\alpha$ and $0$. 

In supply chains, a common objective is to minimize the error between the forecasted inventory and actual inventory, as well as forecasted pipeline and actual pipeline. This objective can be written as 
\begin{equation}\label{eqn:LQ_obj}
    F(i, p, f) = \sum_{t=0}^T\norm{i(t) - \hat{i}(t)}_2^2 + \norm{\ones^\top p - \hat{p}(t)}_2^2 + \norm{o(t)}_2^2. 
\end{equation}
Here $\hat{i}(t)$ and $\hat{p}(t)$ are determined by the demand --- the inventory at time $t$ should satisfy $d(t)$, and the pipeline at time $t$ should supply enough so the inventory at time $t+1$ is non-negative. 
Therefore the LQR formulation is given by 
\[\min_{K}  F(i, p, f)  \text{ s. t. } x(t+1) = Ax(t) - BKx(t) - E d(t). \]
\begin{enumerate}
    \item Typically we do not know $\hat{i}$ and $\hat{p}$ until later. Can this problem be solved with regret minimization?
    \item String stability: when lead time is zero, what is the string stability of a chain of these systems?
\end{enumerate}

\subsection{LTI stability analysis of Supply chain w/out forecast}
We consider the supply chain with a lead time of $1$, no forecasting and a stochastic pipeline, where at every iteration $\alpha \in [0, 1)$ amount of expected product is delayed. 
\begin{equation}\label{eqn:sc_wo_forecast}
    \begin{bmatrix}
        i \\ p
    \end{bmatrix}(t+1) = \begin{bmatrix}
        1 & 1 - \alpha \\
        0 & \alpha
    \end{bmatrix} \begin{bmatrix}
        i \\ p
    \end{bmatrix}(t) + \begin{bmatrix}
        0 \\ 1
    \end{bmatrix} o(t) - \begin{bmatrix}
        1 \\ 0
    \end{bmatrix} d(t)
\end{equation}
\textbf{Natural system response}: the system eigenvalues are given by $(1 - \lambda) (\alpha - \lambda) = 0$: $\lambda = \{1, \alpha\}$. So the system is marginally stable. 

\noindent\textbf{Controllability}: system is controllable if and only if the controllability matrix $[B, AB]$ has full rank. 
\begin{equation}\label{eqn:sc_control_mat}
    \begin{bmatrix}
        B & AB
    \end{bmatrix} = \begin{bmatrix}
        0 & 1 - \alpha \\ 1 & \alpha
    \end{bmatrix}.
\end{equation}
For all $\alpha \in [0, 1)$,~\eqref{eqn:sc_control_mat} is full rank.

\noindent \textbf{Stability}. Given that~\eqref{eqn:sc_wo_forecast} is fully controllable, there exists controllers $K \in \reals^1\times 2$ such that the resulting LTI system is exponentially/asymptotically stable. Furthermore, the origin $[0, 0]$ is an unforced equilibrium point when $d(t) = 0$. 




\subsection{Platoon system}
We consider a single chain supply chain as a platoon system, where the order from supplier $i+1$ $o^i(t)$ is correlated the demand for supplier $i$ $d^i(t)$. 
\begin{equation}
    o^i(t) = d^i(t)
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/supply_chain_connectivity.jpg}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}
For an $N$ supplier supply chain, the total transfer function from a demand $d(t)$ to the inventory of supplier $0$ (last in the chain) $i^0(t)$ is given by 
\begin{equation}
    G(j\omega) = G_{01}(j\omega)G_{12}(j\omega)\ldots G_{(N-2)(N-1)}(j\omega)
\end{equation}
Suppose that each supplier wants to first ensure that their individual transfer function from $o$ to $i$ is stable. This gives us the equilibrium point. 

Then we also should come up with individual conditions on $G_{i(i+1)}(j\omega)$ so that the overall transfer function $G(j\omega)$ is stable. 
Some additional questions - what if I want to minimize the peak gain (what is peak gain)? or the critical damping?

Look into this peak to peak gain control https://arxiv.org/pdf/1903.08599.pdf


\newpage


% \bibliography{reference}

